Characterizing Driving Context from Driver Behavior

Because of the increasing availability of spatiotemporal data, a variety of data-analytic applications have become possible. Characterizing driving context, where context may be thought of as a combination of location and time, is a new challenging application. An example of such a characterization is finding the correlation between driving behavior and traffic conditions. This contextual information enables analysts to validate observation-based hypotheses about the driving of an individual. In this paper, we present DriveContext, a novel framework to find the characteristics of a context, by extracting significant driving patterns (e.g., a slow-down), and then identifying the set of potential causes behind patterns (e.g., traffic congestion). Our experimental results confirm the feasibility of the framework in identifying meaningful driving patterns, with improvements in comparison with the state-of-the-art. We also demonstrate how the framework derives interesting characteristics for different contexts, through real-world examples.

==> DeriveTheContext.tex <==
\label{sec:derive_the_context}
The results of causality analysis provides the strongest signal from which to derive the characteristics for a context. As an example, Figure \ref{fig:physical-facts} shows that one can expect to see about 82\% correlation between driving patterns and physical properties of routes during weekdays, between 3pm to 7pm for Interstate-70. 
Moreover, \sys\ may also be used as an analysis tool for usage-based insurance purposes. As an example, for a given context $c$, the \sys\ may find driving patterns are on average 55\% correlated with physical properties of the route. An insurance company may use such contextual information to study the behavior of an individual driver in order to evaluate how risky or safe he/she is, regarding the characteristics of context $c$. 
The resulting insights from our framework may also be used for driver coaching, which recommends further training to those drivers whose driving behavior in a context is not compatible with the properties of that context.

==> discussion.tex <==
%this section was used previously

\begin{itemize}[leftmargin=*]
    \renewcommand{\labelitemi}{\tiny$\blacksquare$}
    \item Comparison of our approach with state of the art: Regarding the definition of the {\sc dSegment}, the proposed approach is the first solution which takes the behavior of drivers into consideration to segment a trajectory, such that resulting segments demonstrate different patterns of behavior. Our case study (Figures \ref{fig:pmd} and \ref{fig:segmented_trip}) and additional causality analysis may provide more clues to prove this phenomena. More details are provided in Section~\ref{sec:rel}.
    
    \item What the causality analysis suggests? The causality analysis, as described in this study, illustrates three aspects: 1) applicability of the segmentation approach, 2) predictability (interpretability) of the behavior of drivers, and 3) usefulness of \sys\ framework for discovery of characteristics of a context. For the first aspect, we observe that about 74\% of extracted driving patterns are justified by some extrinsic cause. This observation is akin to the measure of {\em precision}\footnote{\scriptsize https://en.wikipedia.org/wiki/Precision\_and\_recall}, which shows how accurate the {\sc dSegment} component is for the extraction of true existing patterns. However, we cannot prove that the remaining 26\% of the extracted patterns are {\em not} related to any extrinsic or intrinsic causes. In addition, we observed how predictable the behavior of a driver is with respect to different situations, such as existence of an intersection, merging into a highway, facing a traffic congestion, etc. Finally, our causality analysis demonstrates how useful \sys\ is as an end-to-end solution for the discovery of driving context from driving patterns. Note that we have mentioned several of contextual properties in terms of insights in previous sub-section. 
    
    \item  How applicable is the \sys\ framework in practice? Regarding the capability of \sys\ as an end-to-end solution, it can be used to study and to explore the context of driving. For example, the application of \sys\ for a given route (context) may find driving patterns are on average 55\% correlated with traffic congestion. 
    An insurance company may use such contextual information to study the behavior of an individual driver in order to find how risky or safe he/she is, regarding the specific context under the study (see Example \ref{ex:UBI}). Besides, leaning about contextual characteristics for different contexts, our system may lead to the discovery of valuable insights about similarities and differences between driving habits for different types of the road, different cities, regions, etc.
\end{itemize}

\sys\ may also provide nuanced insight on driver behavior. For example, we noted that when the focus is on a {\em highway} as the type of the road under study, we observed interesting insights. For instance, in Figure \ref{fig:all}, the coverage of the cutting points of the segments on Interstate 270 is significantly lower than in other routes, during the weekdays. This observation may represent the driving style for Interstate 270 and it may also suggest there is some event or fact that underlies the patterns of driving behavior on this route.
To understand what these events may be, we examined the available Annual Average Daily Traffic (AADT) reports which are provided by Department Of Transportation (DOT) for Columbus, Ohio\footnote{\scriptsize http://www.dot.state.oh.us/Divisions/Planning/TechServ/traffic/Pages/Traffic-Count-Reports-and-Maps.aspx}. Based on these reports for 2010 and 2014 (the most recent ones), as demonstrated by Table \ref{tab:DOT_AADT}, we observed that the proportion of trucks that use Interstate 270 for transportation is significantly larger than for other routes in the test set.
Thus, the presence of truck may be be a potential reason for the difference in the coverage of driving patterns (cutting points) by available extrinsic causes on Interstate 270 in comparison to the other routes in the test set. %the transitions of driving patterns 
Tables \ref{tab:DOT_AADT} also provides the length of the routes and total number of vehicles that use each route as reported by DOT.
Note that for each route in test set, DOT reports just cover a portion of the route that is used in the test set, not the entire route on the map.

\bigskip
\begin{table}[h]
    \centering
    \small
    \caption{\small Annual Average Daily Traffic (AADT) volume estimation for \textbf{2010} and \textbf{2014} for Franklin county of Columbus, OH.}
    \begin{tabular}{c | c | c | c | c | c}
        \textbf{Route} & \textbf{I-70} & \textbf{I-71} & \textbf{I-270} & \textbf{I-670} & \textbf{315 Fwy}\\ [0.6ex]
        \hline
        \textbf{Truck Load (2010)} & 11.5\% & 9.7\% & \textbf{13.5}\% & 5.3\% & 4.3\%\\
        \hline
        \textbf{Truck Load (2014)} & 9.4\% & 8.9\% & \textbf{11.4}\% & 4.9\% & 3.7\%\\
        \hline
        \textbf{Route Length (miles)} & 7.5 & 11.1 & 10.5 & 7.7 & 11.2\\
        \hline
        \textbf{\#Vehicles (millions)} & 1.1 & 1.7 & 1.0 & 1.2 & 1.2\\
    \end{tabular}
    \label{tab:DOT_AADT}
\vspace{-0.1in}
\end{table}

\iffalse
\medskip
\begin{table}[h]
    \centering
    \small
    \caption{\small Annual Average Daily Traffic (AADT) volume estimation for \textbf{2014} for Franklin county of Columbus, OH.}
    \begin{tabular}{c | c | c | c | c | c}
        \textbf{Route} & \textbf{I-70} & \textbf{I-71} & \textbf{I-270} & \textbf{I-670} & \textbf{315 Fwy}\\ [0.6ex]
        \hline
        \textbf{Truck Load-2014\%} & 9.4\% & 8.9\% & \textbf{11.4}\% & 4.9\% & 3.7\%\\
        \hline
        \textbf{Route Length (miles)} & 7.5 & 11.8 & 11.1 & 7.3 & 11.4\\
        \hline
        \textbf{\#Vehicles (millions)} & 0.8 & 1.4 & 0.5 & 1.0 & 1.1\\
    \end{tabular}
    \label{tab:DOT_2014}
    \vspace{-0.08in}
\end{table}
\fi
